Make Some Noise: Reliable and Efficient Single-Step Adversarial Training

Recently, Wong et al. showed that adversarial training with single-step FGSM leads to a characteristic failure mode named Catastrophic Overfitting (CO), in which a model becomes suddenly vulnerable to multi-step attacks. Experimentally they showed that simply adding a random perturbation prior to FGSM (RS-FGSM) could prevent CO. However, Andriushchenko and Flammarion observed that RS-FGSM still leads to CO for larger perturbations, and proposed a computationally expensive regularizer (GradAlign) to avoid it. In this work, we methodically revisit the role of noise and clipping in single-step adversarial training. Contrary to previous intuitions, we find that using a stronger noise around the clean sample combined with \textit{not clipping} is highly effective in avoiding CO for large perturbation radii. We then propose Noise-FGSM (N-FGSM) that, while providing the benefits of single-step adversarial training, does not suffer from CO. Empirical analyses on a large suite of experiments show that N-FGSM is able to match or surpass the performance of previous state-of-the-art GradAlign, while achieving 3x speed-up. Code can be found in https://github.com/pdejorge/N-FGSM

==> Tables/tab_ablation_nfgsm.tex <==
\begin{table*}
\renewcommand{\arraystretch}{1.5}
\centering
\caption{Ablation of the clean and PGD-50-10 accuracy when changing N-FGSM hyperparameters -- noise level $k$ and FGSM step size $\alpha$. Results are averaged over 3 seeds. All models are evaluated with PGD-50-10 attack and $\epsilon_{\textrm{test}} = \epsilon_{\textrm{train}} = 8/255$. \ric{Modified because clean/adv on two different lines per row was not clear. A braplot may be much clearer and space-friendly. TBD}}
\label{table:nfgsm_ablation}
\small
\begin{tabular}{ccccccc}
\toprule
% & \multicolumn{6}{c}{\textbf{Noise level}} \\
% \cmidrule(r){2-7}
           & \multicolumn{2}{c}{$k=0$}  & \multicolumn{2}{c}{$k=1 \epsilon_{\textrm{train}}$} & \multicolumn{2}{c}{$k=2 \epsilon_{\textrm{train}}$} \\
\cmidrule(r){2-3}
\cmidrule(r){4-5}
\cmidrule(r){6-7} 
& Clean & PGD-50-10 & Clean & PGD-50-10 & Clean & PGD-50-10 \\
\midrule
$\alpha = 0$  & 93.8 $\pm$ 0.14 & 0.0 $\pm$ 0.0 & 93.06 $\pm$ 0.02 & 0.0 $\pm$ 0.0    & 91.76 $\pm$ 0.07 & 0.01 $\pm$ 0.0   \\\hline
$\alpha = 4$ & 88.77 $\pm$ 0.04&  35.88 $\pm$ 0.55 & 88.42 $\pm$ 0.03 & 36.7 $\pm$ 0.23  & 87.79 $\pm$ 0.05 & 37.27 $\pm$ 0.23 \\\hline
$\alpha = 6$  & 85.58 $\pm$ 0.11&  43.85 $\pm$ 0.12 & 85.03 $\pm$ 0.09 & 44.44 $\pm$ 0.13 & 84.49 $\pm$ 0.1&  44.44 $\pm$ 0.15  \\\hline
$\alpha = 8$ & 86.41 $\pm$ 0.7   & 0.0 $\pm$ 0.0     & 81.57 $\pm$ 0.07 & 48.16 $\pm$ 0.21 & 80.58 $\pm$ 0.22 & 48.12 $\pm$ 0.07 \\\hline
$\alpha = 10$ & 82.08 $\pm$ 1.62 & 0.0 $\pm$ 0.0    & 77.32 $\pm$ 0.14 & 49.68 $\pm$ 0.25 & 76.49 $\pm$ 0.14 & 49.77 $\pm$ 0.37 \\\hline
$\alpha = 12$ & 80.6 $\pm$ 2.59 &  0.0 $\pm$ 0.0    & 82.0 $\pm$ 1.65 & 0.0 $\pm$ 0.0     & 72.52 $\pm$ 0.16&  50.17 $\pm$ 0.22 \\
\bottomrule
\end{tabular}
\end{table*}

% \begin{table}
% \renewcommand{\arraystretch}{1.2}
% \centering
% \caption{Ablation of the clean (top) and PGD-50-10 (bottom) \ric{top/bottom not clear used like this} accuracy when changing N-FGSM hyperparameters -- noise level $k$ and FGSM step size $\alpha$. Results are averaged over 3 seeds. All models are evaluated with PGD-50-10 attack and $\epsilon_{\textrm{test}} = \epsilon_{\textrm{train}} = 8/255$. \ric{I started modifying, but I think tables are not clear with the two lines per row (clean/adv). TBD, maybe better barplot}}
% \label{table:nfgsm_ablation}
% \small
% \begin{tabular}{cccc}
% \toprule
% & \multicolumn{3}{c}{\textbf{Noise level}} \\
% \cmidrule(r){2-4}
%           & $k=0$  & $k=1 \epsilon_{\textrm{train}}$ & $k=2 \epsilon_{\textrm{train}}$ \\
%           \midrule
% $\alpha = 0$  & 93.8 $\pm$ 0.14 \\ 0.0 $\pm$ 0.0     & 93.06 $\pm$ 0.02 \\ 0.0 $\pm$ 0.0    & 91.76 $\pm$ 0.07 \\ 0.01 $\pm$ 0.0   \\\hline
% $\alpha = 4$ & 88.77 $\pm$ 0.04\\  35.88 $\pm$ 0.55 & 88.42 $\pm$ 0.03 \\ 36.7 $\pm$ 0.23  & 87.79 $\pm$ 0.05 \\ 37.27 $\pm$ 0.23 \\\hline
% $\alpha = 6$  & 85.58 $\pm$ 0.11\\  43.85 $\pm$ 0.12 & 85.03 $\pm$ 0.09 \\ 44.44 $\pm$ 0.13 & 84.49 $\pm$ 0.1\\  44.44 $\pm$ 0.15  \\\hline
% $\alpha = 8$ & 86.41 $\pm$ 0.7   \\ 0.0 $\pm$ 0.0     & 81.57 $\pm$ 0.07 \\ 48.16 $\pm$ 0.21 & 80.58 $\pm$ 0.22 \\ 48.12 $\pm$ 0.07 \\\hline
% $\alpha = 10$ & 82.08 $\pm$ 1.62 \\ 0.0 $\pm$ 0.0    & 77.32 $\pm$ 0.14 \\ 49.68 $\pm$ 0.25 & 76.49 $\pm$ 0.14 \\ 49.77 $\pm$ 0.37 \\\hline
% $\alpha = 12$ & 80.6 $\pm$ 2.59 \\  0.0 $\pm$ 0.0    & 82.0 $\pm$ 1.65 \\ 0.0 $\pm$ 0.0     & 72.52 $\pm$ 0.16\\  50.17 $\pm$ 0.22 \\ \hline
% 
% \end{table}
